A 3D radiative transfer framework: II. line transfer problems

Higher resolution telescopes as well as 3D numerical simulations will require the development of detailed 3D radiative transfer calculations. Building upon our previous work we extend our method to include both continuum and line transfer. We present a general method to calculate radiative transfer including scattering in the continuum as well as in lines in 3D static atmospheres. The scattering problem for line transfer is solved via means of an operator splitting (OS) technique. The formal solution is based on a long-characteristics method. The approximate $\Lambda$ operator is constructed considering nearest neighbors {\em exactly}. The code is parallelized over both wavelength and solid angle using the MPI library. We present the results of several test cases with different values of the thermalization parameter and two choices for the temperature structure. The results are directly compared to 1D spherical tests. With our current grid setup the interior resolution is much lower in 3D than in 1D, nevertheless the 3D results agree very well with the well-tested 1D calculations. We show that with relatively simple parallelization that the code scales to very large number of processors which is mandatory for practical applications. Advances in modern computers will make realistic 3D radiative transfer calculations possible in the near future. Our current code scales to very large numbers of processors, but requires larger memory per processor at high spatial resolution.

==> aa.tex <==
%%==================================================================%%
%%                                                                  %%
%%                                                                  %%
%%                                                                  %%
%%                      A S T R O N O M Y                           %%
%%                                                                  %%
%%                           AND                                    %%
%%                                                                  %%
%%                  A S T R O P H Y S I C S                         %%
%%                                                                  %%
%%                                                                  %%
%%   Plain TeX Support                           Version 2.0, 1991  %%
%%                                                                  %%
%%   This is file AA.TEX the short startup file of the macro        %%
%%   package                                                        %%
%%   Version 2.0 as of 25 Feb 1991                                  %%
%%                                                                  %%
%%==================================================================%%
%
\input aa.cmm
%
%  \refereelayout           % a referee layout
%
  \MAINTITLE={ ????? }      % must be given
%
%
% \FOOTNOTE{ ????? }          \FOOTNOTE is valid only in
%                             \MAINTITLE or in \SUBTITLE
%
  \SUBTITLE={ ????? }       % is optional
%
  \AUTHOR={ ????? }         % Firstname Name<@number><, Nextauthor@number>
%                             items in "<  >" are optional
%                             \PRESADD{Present address} is optional
%
  \INSTITUTE={ ????? }      % Take care of the affiliations used with \AUTHOR
%                             @1 Institute No.1<@2 next institute>
%
  \ABSTRACT={ ????? }       % must be given
%
  \KEYWORDS={ ????? }       % must be given
%
  \THESAURUS={ ????? }      % must be given
%
  \OFFPRINTS={ ????? }      % is optional
%
  \DATE={ ????? }           % must be given at the last moment
%
% Please don't overrule this command, it will format your titlepage.
\maketitle
%
% Now start your text using the Springer macros see the
% instructions in file AA.DOC or the examples in AA.DEM
%
\bye                          % finish your text with this command

